Effectively Sampling Higher Order Mutants Using Causal Effect

Higher Order Mutation (HOM) has been proposed to avoid equivalent mutants and improve the scalability of mutation testing, but generating useful HOMs remain an expensive search problem on its own. We propose a new approach to generate Strongly Subsuming Higher Order Mutants (SSHOM) using a recently introduced Causal Program Dependence Analysis (CPDA). CPDA itself is based on program mutation, and provides quantitative estimation of how often a change of the value of a program element will cause a value change of another program element. Our SSHOM generation approach chooses pairs of program elements using heuristics based on CPDA analysis, performs First Order Mutation to the chosen pairs, and generates an HOM by combining two FOMs.

==> Background.tex <==
%!TEX root=./main.tex

\section{Background}


\subsection*{Higher Order Mutants (HOM)}
Mutants made with mutation operators can be classified by the number of mutation operators applied to the original program. First Order Mutant (FOM) is mutant generated by applying mutation operator once. (definition borrowed) Mutants generated by applying mutation operator more than once are called Higher Order Mutants. 

For HOM $h$, consider set of FOM $F = \{f_1, f_2, \dots, f_n\}$ where each mutant $f_i$ is generated by applying one of mutation operators used to generate $h$. We call the mutants the constituent FOMs of $h$ and say $h$ is consisted of $f_1, f_2, \dots, f_n$. Specifically, second order mutants (SOM) are mutants generated by applying mutation operator twice in original program.

Through lots studies it has been shown that Higher Order Mutation Testing can be used to overcome the \emph{equivalent mutant problem}: The process of deciding whether two mutants are equivalent or not is undecidable problem. Offutt's (reference) empirical study shows that $10\%$ of the first order mutants were found to be equivalent while only $1\%$ of the higher order mutants were. Therefore using HOMs, we are able to solve the equivalent mutant problem to more extent.

Also, the concept of Strongly Higher Order Mutant (SSHOM) encourages us to use HOMs. SSHOM was introduced by Yue Jia. SSHOM are by definition, mutants that are harder to kill than its constituent FOMs.

Let $h$ be a HOM constituted of $\{f_1, f_2, \dots, f_n\}$. Let $T$ a set of test cases and $T_f \subseteq T$ a set of test cases that kills a mutant $f$. We call $h$ is a subsuming mutant if:
\begin{equation}
 |T_h| < |\bigcup_{i}  {T_{f_i} }|
\end{equation}

Applying more strict conditions, mutant $h$ is a strongly subsuming mutant (SSHOM) if: 
\begin{equation}
T_h \subset \bigcap_{i} T_i
\end{equation}
Every test case that kills $h$ should kill all of its constituent first order mutants.

Since $h$ is harder to kill than its constituent FOMs, all constituent mutants of $h$ can be replaced by a $h$ thus decreasing the test effort. For a HOM to be strongly subsuming (subsuming), multiple mutation operations must mask each other. This is because there must exist a test case that all its constituent FOMs gets killed but the higher order mutant lives. 

Now for a set of mutants $M = \{m_1, m_2, \dots , m_k\}$ strongly subsuming rate (subsuming rate) of M is calculated as follows.
\begin{equation}
    SSR(M) = \frac{|SSHOM(M)|}{|M|}
\end{equation}
Where $SSHOM(M)$ is the set of mutants in $M$ that are strongly subsuming.

\subsubsection*{Diversity of Mutants}
Another important feature to look for when sampling mutants is the diversity. Since the purpose of each mutant are made to mimic real faults of developers, we always want more diverse mutants. To define the diversity metric, we first introduce the kill vector of a mutant.

For a mutant $m$ of original program $P$ with test suite $T$, a kill vector $v \in \mathcal{R}^|T|$ of $m$ is defined as follows.
\begin{equation*}
  v_i =
  \begin{cases}
    1
    &
    \text{if $T_i$ kills $m$;}
    \\[10pt]
    0
    &
    \text{otherwise.}
  \end{cases}
\end{equation*}
where $T_i$ refers to $i$-th test case of $T$. ($1 \le i \le |T|$)

The diversity of set of mutants $M = \{m_1, m_2, \dots, m_k\}$ is then defined as follows.
\begin{equation}
    dScore(M) = \frac{|\{v_1, v_2, \dots \}|}{|M|}
\end{equation}
where $v_i$ is the kill vector of $m_i$.

Note here that higher $dScore$ is achieved if certain set of mutants contain more mutants with distinct kill vectors. The reason we define diversity with kill vectors is because two mutants with same kill vectors are not distinguishable from the point of test suite. Yet if the two mutants have different kill vectors, we know for sure that the two mutants have different faults.

==> Future_Works.tex <==
%!TEX root=./main.tex

\section{Future Works}

